Morpheus: Text-Driven 3D Gaussian Splat Shape and Color Stylization

Exploring real-world spaces using novel-view synthesis is fun, and reimagining those worlds in a different style adds another layer of excitement. Stylized worlds can also be used for downstream tasks where there is limited training data and a need to expand a model's training distribution. Most current novel-view synthesis stylization techniques lack the ability to convincingly change geometry. This is because any geometry change requires increased style strength which is often capped for stylization stability and consistency. In this work, we propose a new autoregressive 3D Gaussian Splatting stylization method. As part of this method, we contribute a new RGBD diffusion model that allows for strength control over appearance and shape stylization. To ensure consistency across stylized frames, we use a combination of novel depth-guided cross attention, feature injection, and a Warp ControlNet conditioned on composite frames for guiding the stylization of new frames. We validate our method via extensive qualitative results, quantitative experiments, and a user study. Code online.

==> figures/comparisons_figure/comparisons_transposed_2.tex <==
\setlength\tabcolsep{0pt}
\renewcommand{\arraystretch}{0}
\begin{tabular}{ccccccc}
    \centering
     & Original & GaussCtrl~\cite{wu2024gaussctrl} & instruct-gs2gs~\cite{vachha2024instruct} & instruct-n2n~\cite{haque2023instruct} & DGE~\cite{chen2024dge} & Ours \\
     

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ snowman on a \\ table in the \\ garden in the \\ snow}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_8068231096698225420_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_8068231096698225420_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_8068231096698225420_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_8068231096698225420_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_8068231096698225420_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_8068231096698225420_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ halloween \\ garden with \\ pumpkins}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_9032712464155832933_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_9032712464155832933_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_9032712464155832933_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_9032712464155832933_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_9032712464155832933_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_9032712464155832933_ours.jpg}
    % \\

    \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ fountain in the \\ desert}}}}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_a_photo_of_a_fountain_in_the_desert_original.jpg}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_a_photo_of_a_fountain_in_the_desert_gaussctrl.jpg}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_a_photo_of_a_fountain_in_the_desert_instruct_gs2gs.jpg}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_a_photo_of_a_fountain_in_the_desert_instruct_nerf2nerf.jpg}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_a_photo_of_a_fountain_in_the_desert_DGE.jpg}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_a_photo_of_a_fountain_in_the_desert_ours.jpg}
    \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{a Picasso \\ painting of a \\ microbiology \\ laboratory with \\ microscopes at \\ a university}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_7216997967437376577_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_7216997967437376577_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_7216997967437376577_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_7216997967437376577_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_7216997967437376577_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_7216997967437376577_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{an Edvard Munch \\ painting of a \\ microbiology \\ laboratory with \\ microscopes at \\ a university}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_5957124393565218005_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_5957124393565218005_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_5957124393565218005_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_5957124393565218005_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_5957124393565218005_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_5957124393565218005_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{Steampunk \\ laboratory with \\ brass \\ instruments, \\ gears, and \\ retro \\ scientific \\ equipment}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_3892785080578390569_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_3892785080578390569_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_3892785080578390569_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_3892785080578390569_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_3892785080578390569_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_3892785080578390569_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{Medieval \\ herbalist lab \\ with dried \\ plants, wooden \\ tables, and \\ candle lighting}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_4481745152940055895_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_4481745152940055895_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_4481745152940055895_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_4481745152940055895_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_4481745152940055895_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_4481745152940055895_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{Ancient \\ alchemist's lab \\ with potion \\ bottles, \\ parchment, and \\ mystical \\ symbols}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_6010283219551870001_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_6010283219551870001_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_6010283219551870001_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_6010283219551870001_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_6010283219551870001_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_6010283219551870001_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{a \\ near-futuristic \\ night city \\ Cyberpunk2077 \\ style picture \\ of a robotics \\ laboratory with \\ computers and a \\ sofa at a \\ university}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6296494377432347600_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6296494377432347600_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6296494377432347600_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6296494377432347600_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6296494377432347600_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6296494377432347600_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{a Picasso \\ painting of a \\ robotics \\ laboratory with \\ computers and a \\ sofa at a \\ university}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_9174672892780308957_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_9174672892780308957_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_9174672892780308957_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_9174672892780308957_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_9174672892780308957_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_9174672892780308957_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{a Van Gogh \\ painting of a \\ robotics \\ laboratory with \\ computers and a \\ sofa at a \\ university}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4872988999019657393_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4872988999019657393_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4872988999019657393_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4872988999019657393_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4872988999019657393_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4872988999019657393_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{Retro arcade \\ room with \\ classic game \\ machines, \\ colorful \\ lights, and \\ vintage posters}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_2425453735404758992_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_2425453735404758992_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_2425453735404758992_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_2425453735404758992_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_2425453735404758992_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_2425453735404758992_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{Jungle-themed \\ break room with \\ plants, natural \\ wood furniture, \\ and tropical \\ decor}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4336440483597926783_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4336440483597926783_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4336440483597926783_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4336440483597926783_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4336440483597926783_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4336440483597926783_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{Medieval tavern \\ with wooden \\ tables, stone \\ walls, and \\ candle lighting}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6792325757249564920_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6792325757249564920_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6792325757249564920_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6792325757249564920_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6792325757249564920_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6792325757249564920_ours.jpg}
    % \\

    \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{Minimalist \\ Japanese tea \\ room with \\ tatami mats, \\ low wooden \\ tables, and \\ paper lanterns}}}}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_8434808770058320497_original.jpg}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_8434808770058320497_gaussctrl.jpg}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_8434808770058320497_instruct_gs2gs.jpg}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_8434808770058320497_instruct_nerf2nerf.jpg}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_8434808770058320497_DGE.jpg}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_8434808770058320497_ours.jpg}
    \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{Victorian \\ parlor with \\ ornate \\ furniture, dark \\ wallpaper, and \\ chandeliers}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_3917677443825827236_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_3917677443825827236_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_3917677443825827236_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_3917677443825827236_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_3917677443825827236_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_3917677443825827236_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{1950s \\ diner-style \\ lounge with \\ checkered \\ floors, red \\ vinyl seats, \\ and jukebox}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_7607527627453949069_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_7607527627453949069_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_7607527627453949069_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_7607527627453949069_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_7607527627453949069_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_7607527627453949069_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{Modern art \\ studio with \\ paint \\ splatters, \\ canvases, and \\ abstract \\ sculptures}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6124102173073698624_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6124102173073698624_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6124102173073698624_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6124102173073698624_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6124102173073698624_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6124102173073698624_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{a Fauvism \\ painting of a \\ photo of a \\ conference room \\ with tables and \\ chairs}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_f_conference_2614162896365812929_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_f_conference_2614162896365812929_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_f_conference_2614162896365812929_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_f_conference_2614162896365812929_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_f_conference_2614162896365812929_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_f_conference_2614162896365812929_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{a Hiroshige \\ Utagawa \\ painting of a \\ kitchen}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_h_kitchen_7313597891086098452_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_h_kitchen_7313597891086098452_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_h_kitchen_7313597891086098452_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_h_kitchen_7313597891086098452_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_h_kitchen_7313597891086098452_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_h_kitchen_7313597891086098452_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{a Bastion game \\ style picture \\ of a flat with \\ a bathroom, \\ living room and \\ a kitchen}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_i_bathroom_2463265628774932085_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_i_bathroom_2463265628774932085_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_i_bathroom_2463265628774932085_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_i_bathroom_2463265628774932085_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_i_bathroom_2463265628774932085_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_i_bathroom_2463265628774932085_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ robot dinosaur \\ on the road \\ side}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_3038377324408634801_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_3038377324408634801_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_3038377324408634801_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_3038377324408634801_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_3038377324408634801_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_3038377324408634801_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{a photo of an \\ ostrich at a \\ farm}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_an_ostrich_at_a_farm_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_an_ostrich_at_a_farm_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_an_ostrich_at_a_farm_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_an_ostrich_at_a_farm_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_an_ostrich_at_a_farm_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_an_ostrich_at_a_farm_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ giraffe on a \\ desert}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_a_giraffe_on_a_desert_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_a_giraffe_on_a_desert_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_a_giraffe_on_a_desert_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_a_giraffe_on_a_desert_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_a_giraffe_on_a_desert_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_a_giraffe_on_a_desert_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ giraffe in zoo}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_giraffe_in_zoo_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_giraffe_in_zoo_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_giraffe_in_zoo_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_giraffe_in_zoo_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_giraffe_in_zoo_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_giraffe_in_zoo_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ medieval horse \\ in front of the \\ castle}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_6128427055822205356_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_6128427055822205356_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_6128427055822205356_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_6128427055822205356_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_6128427055822205356_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_6128427055822205356_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ cyberpunk sci \\ robot horse}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_cyberpunk_sci_robot_horse_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_cyberpunk_sci_robot_horse_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_cyberpunk_sci_robot_horse_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_cyberpunk_sci_robot_horse_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_cyberpunk_sci_robot_horse_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_cyberpunk_sci_robot_horse_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{Photo of a \\ dinosaur}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Photo_of_a_dinosaur_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Photo_of_a_dinosaur_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Photo_of_a_dinosaur_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Photo_of_a_dinosaur_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Photo_of_a_dinosaur_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Photo_of_a_dinosaur_ours.jpg}
    % \\

    \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{Cubist portrait \\ of a horse}}}}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Cubist_portrait_of_a_horse_original.jpg}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Cubist_portrait_of_a_horse_gaussctrl.jpg}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Cubist_portrait_of_a_horse_instruct_gs2gs.jpg}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Cubist_portrait_of_a_horse_instruct_nerf2nerf.jpg}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Cubist_portrait_of_a_horse_DGE.jpg}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Cubist_portrait_of_a_horse_ours.jpg}
    \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{Steampunk horse \\ statue with \\ brass gears, \\ pipes, and \\ mechanical \\ parts}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1620797878807124195_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1620797878807124195_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1620797878807124195_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1620797878807124195_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1620797878807124195_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1620797878807124195_ours.jpg}
    % \\

    \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{Horse statue \\ made from \\ stacked wooden \\ blocks, rustic \\ and \\ minimalistic}}}}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_4477867171741382541_original.jpg}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_4477867171741382541_gaussctrl.jpg}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_4477867171741382541_instruct_gs2gs.jpg}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_4477867171741382541_instruct_nerf2nerf.jpg}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_4477867171741382541_DGE.jpg}
    & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_4477867171741382541_ours.jpg}
    \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{Horse statue \\ made from very \\ large lego \\ bricks in front \\ of a museum}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1883532210605779899_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1883532210605779899_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1883532210605779899_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1883532210605779899_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1883532210605779899_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1883532210605779899_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{80s retro car \\ on a neon grid \\ landscape with \\ pink and blue \\ glowing lights}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6784128519023507286_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6784128519023507286_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6784128519023507286_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6784128519023507286_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6784128519023507286_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6784128519023507286_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{Monster truck \\ car with \\ oversized \\ wheels and a \\ lifted body}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_5687717264768732369_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_5687717264768732369_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_5687717264768732369_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_5687717264768732369_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_5687717264768732369_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_5687717264768732369_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{Tank with \\ treads and \\ heavy armor in \\ a rugged \\ environment}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6799381787614477972_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6799381787614477972_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6799381787614477972_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6799381787614477972_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6799381787614477972_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6799381787614477972_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{Photo of a tron \\ legacy \\ nightrider neon \\ futuristic \\ night}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_3698942648060598118_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_3698942648060598118_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_3698942648060598118_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_3698942648060598118_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_3698942648060598118_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_3698942648060598118_ours.jpg}
    % \\

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ Batmobile}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_photo_of_a_Batmobile_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_photo_of_a_Batmobile_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_photo_of_a_Batmobile_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_photo_of_a_Batmobile_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_photo_of_a_Batmobile_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_photo_of_a_Batmobile_ours.jpg}
    % \\2

    % \raisebox{1.5\height}{\parbox[t]{15mm}{\rotatebox[origin=c]{90}{\makecell{a screenshot of \\ a Minecraft car}}}}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_screenshot_of_a_Minecraft_car_original.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_screenshot_of_a_Minecraft_car_gaussctrl.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_screenshot_of_a_Minecraft_car_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_screenshot_of_a_Minecraft_car_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_screenshot_of_a_Minecraft_car_DGE.jpg}
    % & \includegraphics[width=0.13333333333333333\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_screenshot_of_a_Minecraft_car_ours.jpg}
    % \\

\end{tabular}


==> figures/comparisons_figure/comparisons_transposed_supp_3.tex <==
\setlength\tabcolsep{0pt}
\renewcommand{\arraystretch}{0}
\begin{tabular}{ccccccc}
    \centering

     & Original & GaussCtrl~\cite{wu2024gaussctrl} & Instruct-GS2GS~\cite{vachha2024instruct} & Instruct-N2N~\cite{haque2023instruct} & DGE~\cite{chen2024dge} & Ours \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ polar bear in \\ the winter forest}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_6210971389578005099_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_6210971389578005099_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_6210971389578005099_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_6210971389578005099_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_6210971389578005099_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_6210971389578005099_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{8mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ human skeleton}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_908885612315295561_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_908885612315295561_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_908885612315295561_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_908885612315295561_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_908885612315295561_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_908885612315295561_ours.jpg}
%     % \\



%     % \raisebox{1.3\height}{\parbox[t]{8mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ chimp}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_a_photo_of_a_chimp_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_a_photo_of_a_chimp_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_a_photo_of_a_chimp_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_a_photo_of_a_chimp_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_a_photo_of_a_chimp_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_a_photo_of_a_chimp_ours.jpg}
%     % \\


%     % \raisebox{1.0\height}{\parbox[t]{8mm}{\rotatebox[origin=c]{90}{\makecell{a photo of the \\ face of the Hulk}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_a_photo_of_the_face_of_the_Hulk_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_a_photo_of_the_face_of_the_Hulk_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_a_photo_of_the_face_of_the_Hulk_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_a_photo_of_the_face_of_the_Hulk_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_a_photo_of_the_face_of_the_Hulk_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_a_photo_of_the_face_of_the_Hulk_ours.jpg}
%     % \\


%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ fountain in the \\ desert}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_a_photo_of_a_fountain_in_the_desert_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_a_photo_of_a_fountain_in_the_desert_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_a_photo_of_a_fountain_in_the_desert_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_a_photo_of_a_fountain_in_the_desert_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_a_photo_of_a_fountain_in_the_desert_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_a_photo_of_a_fountain_in_the_desert_ours.jpg}
%     % \\


%     % \raisebox{1.2\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Minimalist \\ Japanese tea \\ room  }}}}
%     % %with \\ tatami mats, \\ low wooden \\ tables, and \\ paper lanterns
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_8434808770058320497_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_8434808770058320497_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_8434808770058320497_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_8434808770058320497_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_8434808770058320497_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_8434808770058320497_ours.jpg}
%     % \\


%     % \raisebox{1.05\height}{\parbox[t]{8mm}{\rotatebox[origin=c]{90}{\makecell{Cubist portrait \\ of a horse}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Cubist_portrait_of_a_horse_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Cubist_portrait_of_a_horse_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Cubist_portrait_of_a_horse_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Cubist_portrait_of_a_horse_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Cubist_portrait_of_a_horse_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Cubist_portrait_of_a_horse_ours.jpg}
%     % \\



%     % \raisebox{0.85\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Horse statue \\ made from stacked \\ wooden blocks}}}}
%     % % \\ blocks, rustic \\ and \\ minimalistic
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_4477867171741382541_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_4477867171741382541_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_4477867171741382541_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_4477867171741382541_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_4477867171741382541_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_4477867171741382541_ours.jpg}
%     % \\

% %%%%%%%%%%%%%%%%%%%

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ hippopotamus \\ next to a river}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_4117844308982924486_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_4117844308982924486_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_4117844308982924486_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_4117844308982924486_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_4117844308982924486_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_4117844308982924486_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ panda in the \\ bamboo forest}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_a_photo_of_a_panda_in_the_bamboo_forest_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_a_photo_of_a_panda_in_the_bamboo_forest_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_a_photo_of_a_panda_in_the_bamboo_forest_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_a_photo_of_a_panda_in_the_bamboo_forest_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_a_photo_of_a_panda_in_the_bamboo_forest_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_a_photo_of_a_panda_in_the_bamboo_forest_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ rhino}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_a_photo_of_a_rhino_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_a_photo_of_a_rhino_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_a_photo_of_a_rhino_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_a_photo_of_a_rhino_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_a_photo_of_a_rhino_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bear_a_photo_of_a_rhino_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ face of a man \\ with a \\ moustache}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_8017864593733457894_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_8017864593733457894_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_8017864593733457894_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_8017864593733457894_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_8017864593733457894_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_8017864593733457894_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ man wearing a \\ pair of glasses}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_1626588165611913311_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_1626588165611913311_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_1626588165611913311_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_1626588165611913311_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_1626588165611913311_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_1626588165611913311_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ face of an old \\ man with \\ wrinkles}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_6901936895449565284_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_6901936895449565284_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_6901936895449565284_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_6901936895449565284_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_6901936895449565284_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_6901936895449565284_ours.jpg}
%     % \\


%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ face with a hat \\ on}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_a_photo_of_a_face_with_a_hat_on_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_a_photo_of_a_face_with_a_hat_on_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_a_photo_of_a_face_with_a_hat_on_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_a_photo_of_a_face_with_a_hat_on_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_a_photo_of_a_face_with_a_hat_on_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/fangzhou_a_photo_of_a_face_with_a_hat_on_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ face of a man \\ with a \\ moustache}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_8017864593733457894_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_8017864593733457894_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_8017864593733457894_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_8017864593733457894_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_8017864593733457894_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_8017864593733457894_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ man wearing a \\ pair of glasses}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_1626588165611913311_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_1626588165611913311_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_1626588165611913311_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_1626588165611913311_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_1626588165611913311_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_1626588165611913311_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ face of an old \\ man with \\ wrinkles}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_6901936895449565284_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_6901936895449565284_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_6901936895449565284_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_6901936895449565284_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_6901936895449565284_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_6901936895449565284_ours.jpg}
%     % \\

%     %%%%%

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ man wearing \\ steampunk \\ goggles}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_7815010103953380534_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_7815010103953380534_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_7815010103953380534_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_7815010103953380534_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_7815010103953380534_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_7815010103953380534_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ face with a hat \\ on}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_a_photo_of_a_face_with_a_hat_on_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_a_photo_of_a_face_with_a_hat_on_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_a_photo_of_a_face_with_a_hat_on_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_a_photo_of_a_face_with_a_hat_on_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_a_photo_of_a_face_with_a_hat_on_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_a_photo_of_a_face_with_a_hat_on_ours.jpg}
%     % \\
%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Portrait of a \\ 19th-century \\ aristocrat with \\ a powdered wig \\ and elaborate \\ clothing}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_4165614350096215214_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_4165614350096215214_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_4165614350096215214_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_4165614350096215214_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_4165614350096215214_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_4165614350096215214_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Viking warrior \\ portrait with a \\ braided beard, \\ fur cloak, and \\ a fierce \\ expression}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_5123690070715721174_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_5123690070715721174_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_5123690070715721174_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_5123690070715721174_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_5123690070715721174_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/face_5123690070715721174_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ snowman on a \\ table in the \\ garden in the \\ snow}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_8068231096698225420_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_8068231096698225420_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_8068231096698225420_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_8068231096698225420_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_8068231096698225420_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_8068231096698225420_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ halloween \\ garden with \\ pumpkins}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_9032712464155832933_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_9032712464155832933_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_9032712464155832933_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_9032712464155832933_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_9032712464155832933_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_9032712464155832933_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ fountain in the \\ desert}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_a_photo_of_a_fountain_in_the_desert_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_a_photo_of_a_fountain_in_the_desert_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_a_photo_of_a_fountain_in_the_desert_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_a_photo_of_a_fountain_in_the_desert_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_a_photo_of_a_fountain_in_the_desert_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_a_photo_of_a_fountain_in_the_desert_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a Picasso \\ painting of a \\ microbiology \\ laboratory with \\ microscopes at \\ a university}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_7216997967437376577_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_7216997967437376577_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_7216997967437376577_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_7216997967437376577_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_7216997967437376577_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_7216997967437376577_ours.jpg}
%     % \\

%     % % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{an Edvard Munch \\ painting of a \\ microbiology \\ laboratory with \\ microscopes at \\ a university}}}}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_5957124393565218005_original.jpg}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_5957124393565218005_gaussctrl.jpg}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_5957124393565218005_instruct_gs2gs.jpg}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_5957124393565218005_instruct_nerf2nerf.jpg}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_5957124393565218005_DGE.jpg}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_5957124393565218005_ours.jpg}
%     % % \\

%     % % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Steampunk \\ laboratory with \\ brass \\ instruments, \\ gears, and \\ retro \\ scientific \\ equipment}}}}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_3892785080578390569_original.jpg}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_3892785080578390569_gaussctrl.jpg}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_3892785080578390569_instruct_gs2gs.jpg}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_3892785080578390569_instruct_nerf2nerf.jpg}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_3892785080578390569_DGE.jpg}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_3892785080578390569_ours.jpg}
%     % % \\

%     % % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Medieval \\ herbalist lab \\ with dried \\ plants, wooden \\ tables, and \\ candle lighting}}}}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_4481745152940055895_original.jpg}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_4481745152940055895_gaussctrl.jpg}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_4481745152940055895_instruct_gs2gs.jpg}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_4481745152940055895_instruct_nerf2nerf.jpg}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_4481745152940055895_DGE.jpg}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_4481745152940055895_ours.jpg}
%     % % \\

%     % %%%%

%     % % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Ancient \\ alchemist's lab \\ with potion \\ bottles, \\ parchment, and \\ mystical \\ symbols}}}}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_6010283219551870001_original.jpg}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_6010283219551870001_gaussctrl.jpg}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_6010283219551870001_instruct_gs2gs.jpg}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_6010283219551870001_instruct_nerf2nerf.jpg}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_6010283219551870001_DGE.jpg}
%     % % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_6010283219551870001_ours.jpg}
%     % % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a \\ near-futuristic \\ night city \\ Cyberpunk2077 \\ style picture \\ of a robotics \\ laboratory with \\ computers and a \\ sofa at a \\ university}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6296494377432347600_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6296494377432347600_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6296494377432347600_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6296494377432347600_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6296494377432347600_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6296494377432347600_ours.jpg}
%     % \\

%     %%%%%

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a Picasso \\ painting of a \\ robotics \\ laboratory with \\ computers and a \\ sofa at a \\ university}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_9174672892780308957_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_9174672892780308957_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_9174672892780308957_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_9174672892780308957_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_9174672892780308957_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_9174672892780308957_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a Van Gogh \\ painting of a \\ robotics \\ laboratory with \\ computers and a \\ sofa at a \\ university}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4872988999019657393_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4872988999019657393_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4872988999019657393_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4872988999019657393_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4872988999019657393_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4872988999019657393_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Retro arcade \\ room with \\ classic game \\ machines, \\ colorful \\ lights, and \\ vintage posters}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_2425453735404758992_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_2425453735404758992_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_2425453735404758992_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_2425453735404758992_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_2425453735404758992_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_2425453735404758992_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Jungle-themed \\ break room with \\ plants, natural \\ wood furniture, \\ and tropical \\ decor}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4336440483597926783_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4336440483597926783_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4336440483597926783_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4336440483597926783_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4336440483597926783_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4336440483597926783_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Medieval tavern \\ with wooden \\ tables, stone \\ walls, and \\ candle lighting}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6792325757249564920_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6792325757249564920_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6792325757249564920_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6792325757249564920_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6792325757249564920_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6792325757249564920_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Minimalist \\ Japanese tea \\ room with \\ tatami mats, \\ low wooden \\ tables, and \\ paper lanterns}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_8434808770058320497_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_8434808770058320497_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_8434808770058320497_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_8434808770058320497_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_8434808770058320497_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_8434808770058320497_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Victorian \\ parlor with \\ ornate \\ furniture, dark \\ wallpaper, and \\ chandeliers}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_3917677443825827236_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_3917677443825827236_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_3917677443825827236_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_3917677443825827236_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_3917677443825827236_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_3917677443825827236_ours.jpg}
%     % \\

%     %%

%     \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{1950s \\ diner-style \\ lounge with \\ checkered \\ floors, red \\ vinyl seats, \\ and jukebox}}}}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_7607527627453949069_original.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_7607527627453949069_gaussctrl.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_7607527627453949069_instruct_gs2gs.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_7607527627453949069_instruct_nerf2nerf.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_7607527627453949069_DGE.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_7607527627453949069_ours.jpg}
%     \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Modern art \\ studio with \\ paint \\ splatters, \\ canvases, and \\ abstract \\ sculptures}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6124102173073698624_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6124102173073698624_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6124102173073698624_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6124102173073698624_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6124102173073698624_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6124102173073698624_ours.jpg}
%     % \\

%     \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a Fauvism \\ painting of a \\ photo of a \\ conference room \\ with tables and \\ chairs}}}}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_f_conference_2614162896365812929_original.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_f_conference_2614162896365812929_gaussctrl.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_f_conference_2614162896365812929_instruct_gs2gs.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_f_conference_2614162896365812929_instruct_nerf2nerf.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_f_conference_2614162896365812929_DGE.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_f_conference_2614162896365812929_ours.jpg}
%     \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a Hiroshige \\ Utagawa \\ painting of a \\ kitchen}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_h_kitchen_7313597891086098452_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_h_kitchen_7313597891086098452_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_h_kitchen_7313597891086098452_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_h_kitchen_7313597891086098452_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_h_kitchen_7313597891086098452_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_h_kitchen_7313597891086098452_ours.jpg}
%     % \\

%     \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a Bastion game \\ style picture \\ of a flat with \\ a bathroom, \\ living room and \\ a kitchen}}}}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_i_bathroom_2463265628774932085_original.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_i_bathroom_2463265628774932085_gaussctrl.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_i_bathroom_2463265628774932085_instruct_gs2gs.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_i_bathroom_2463265628774932085_instruct_nerf2nerf.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_i_bathroom_2463265628774932085_DGE.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_i_bathroom_2463265628774932085_ours.jpg}
%     \\

%     \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ robot dinosaur \\ on the road \\ side}}}}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_3038377324408634801_original.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_3038377324408634801_gaussctrl.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_3038377324408634801_instruct_gs2gs.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_3038377324408634801_instruct_nerf2nerf.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_3038377324408634801_DGE.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_3038377324408634801_ours.jpg}
%     \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of an \\ ostrich at a \\ farm}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_an_ostrich_at_a_farm_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_an_ostrich_at_a_farm_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_an_ostrich_at_a_farm_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_an_ostrich_at_a_farm_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_an_ostrich_at_a_farm_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_an_ostrich_at_a_farm_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ giraffe on a \\ desert}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_a_giraffe_on_a_desert_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_a_giraffe_on_a_desert_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_a_giraffe_on_a_desert_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_a_giraffe_on_a_desert_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_a_giraffe_on_a_desert_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_a_giraffe_on_a_desert_ours.jpg}
%     % \\

%     \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ giraffe in zoo}}}}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_giraffe_in_zoo_original.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_giraffe_in_zoo_gaussctrl.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_giraffe_in_zoo_instruct_gs2gs.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_giraffe_in_zoo_instruct_nerf2nerf.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_giraffe_in_zoo_DGE.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_giraffe_in_zoo_ours.jpg}
%     \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ medieval horse \\ in front of the \\ castle}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_6128427055822205356_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_6128427055822205356_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_6128427055822205356_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_6128427055822205356_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_6128427055822205356_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_6128427055822205356_ours.jpg}
%     % \\

%     \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ cyberpunk sci \\ robot horse}}}}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_cyberpunk_sci_robot_horse_original.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_cyberpunk_sci_robot_horse_gaussctrl.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_cyberpunk_sci_robot_horse_instruct_gs2gs.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_cyberpunk_sci_robot_horse_instruct_nerf2nerf.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_cyberpunk_sci_robot_horse_DGE.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_cyberpunk_sci_robot_horse_ours.jpg}
%     \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Photo of a \\ dinosaur}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Photo_of_a_dinosaur_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Photo_of_a_dinosaur_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Photo_of_a_dinosaur_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Photo_of_a_dinosaur_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Photo_of_a_dinosaur_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Photo_of_a_dinosaur_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Cubist portrait \\ of a horse}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Cubist_portrait_of_a_horse_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Cubist_portrait_of_a_horse_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Cubist_portrait_of_a_horse_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Cubist_portrait_of_a_horse_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Cubist_portrait_of_a_horse_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Cubist_portrait_of_a_horse_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Steampunk horse \\ statue with \\ brass gears, \\ pipes, and \\ mechanical \\ parts}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1620797878807124195_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1620797878807124195_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1620797878807124195_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1620797878807124195_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1620797878807124195_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1620797878807124195_ours.jpg}
%     % \\

%     \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Horse statue \\ made from \\ stacked wooden \\ blocks, rustic \\ and \\ minimalistic}}}}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_4477867171741382541_original.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_4477867171741382541_gaussctrl.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_4477867171741382541_instruct_gs2gs.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_4477867171741382541_instruct_nerf2nerf.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_4477867171741382541_DGE.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_4477867171741382541_ours.jpg}
%     \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Horse statue \\ made from very \\ large lego \\ bricks in front \\ of a museum}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1883532210605779899_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1883532210605779899_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1883532210605779899_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1883532210605779899_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1883532210605779899_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1883532210605779899_ours.jpg}
%     % \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{80s retro car \\ on a neon grid \\ landscape with \\ pink and blue \\ glowing lights}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6784128519023507286_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6784128519023507286_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6784128519023507286_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6784128519023507286_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6784128519023507286_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6784128519023507286_ours.jpg}
%     % \\

%     \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Monster truck \\ car with \\ oversized \\ wheels and a \\ lifted body}}}}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_5687717264768732369_original.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_5687717264768732369_gaussctrl.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_5687717264768732369_instruct_gs2gs.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_5687717264768732369_instruct_nerf2nerf.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_5687717264768732369_DGE.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_5687717264768732369_ours.jpg}
%     \\

%     % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Tank with \\ treads and \\ heavy armor in \\ a rugged \\ environment}}}}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6799381787614477972_original.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6799381787614477972_gaussctrl.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6799381787614477972_instruct_gs2gs.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6799381787614477972_instruct_nerf2nerf.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6799381787614477972_DGE.jpg}
%     % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6799381787614477972_ours.jpg}
%     % \\

%     \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Photo of a tron \\ legacy \\ nightrider neon \\ futuristic \\ night}}}}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_3698942648060598118_original.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_3698942648060598118_gaussctrl.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_3698942648060598118_instruct_gs2gs.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_3698942648060598118_instruct_nerf2nerf.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_3698942648060598118_DGE.jpg}
%     & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_3698942648060598118_ours.jpg}
%     \\

    \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ Batmobile}}}}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_photo_of_a_Batmobile_original.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_photo_of_a_Batmobile_gaussctrl.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_photo_of_a_Batmobile_instruct_gs2gs.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_photo_of_a_Batmobile_instruct_nerf2nerf.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_photo_of_a_Batmobile_DGE.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_photo_of_a_Batmobile_ours.jpg}
    \\

    \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a screenshot of \\ a Minecraft car}}}}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_screenshot_of_a_Minecraft_car_original.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_screenshot_of_a_Minecraft_car_gaussctrl.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_screenshot_of_a_Minecraft_car_instruct_gs2gs.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_screenshot_of_a_Minecraft_car_instruct_nerf2nerf.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_screenshot_of_a_Minecraft_car_DGE.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_screenshot_of_a_Minecraft_car_ours.jpg}
    \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ snowman on a \\ table in the \\ garden in the \\ snow}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_8068231096698225420_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_8068231096698225420_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_8068231096698225420_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_8068231096698225420_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_8068231096698225420_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_8068231096698225420_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ halloween \\ garden with \\ pumpkins}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_9032712464155832933_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_9032712464155832933_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_9032712464155832933_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_9032712464155832933_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_9032712464155832933_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/mipnerf_garden_9032712464155832933_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a Picasso \\ painting of a \\ microbiology \\ laboratory with \\ microscopes at \\ a university}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_7216997967437376577_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_7216997967437376577_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_7216997967437376577_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_7216997967437376577_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_7216997967437376577_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_7216997967437376577_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{an Edvard Munch \\ painting of a \\ microbiology \\ laboratory with \\ microscopes at \\ a university}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_5957124393565218005_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_5957124393565218005_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_5957124393565218005_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_5957124393565218005_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_5957124393565218005_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_5957124393565218005_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Steampunk \\ laboratory with \\ brass \\ instruments, \\ gears, and \\ retro \\ scientific \\ equipment}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_3892785080578390569_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_3892785080578390569_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_3892785080578390569_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_3892785080578390569_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_3892785080578390569_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_3892785080578390569_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Medieval \\ herbalist lab \\ with dried \\ plants, wooden \\ tables, and \\ candle lighting}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_4481745152940055895_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_4481745152940055895_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_4481745152940055895_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_4481745152940055895_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_4481745152940055895_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_4481745152940055895_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Ancient \\ alchemist's lab \\ with potion \\ bottles, \\ parchment, and \\ mystical \\ symbols}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_6010283219551870001_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_6010283219551870001_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_6010283219551870001_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_6010283219551870001_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_6010283219551870001_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_a_microscopes_6010283219551870001_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a \\ near-futuristic \\ night city \\ Cyberpunk2077 \\ style picture \\ of a robotics \\ laboratory with \\ computers and a \\ sofa at a \\ university}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6296494377432347600_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6296494377432347600_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6296494377432347600_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6296494377432347600_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6296494377432347600_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6296494377432347600_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a Picasso \\ painting of a \\ robotics \\ laboratory with \\ computers and a \\ sofa at a \\ university}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_9174672892780308957_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_9174672892780308957_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_9174672892780308957_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_9174672892780308957_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_9174672892780308957_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_9174672892780308957_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a Van Gogh \\ painting of a \\ robotics \\ laboratory with \\ computers and a \\ sofa at a \\ university}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4872988999019657393_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4872988999019657393_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4872988999019657393_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4872988999019657393_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4872988999019657393_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4872988999019657393_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Retro arcade \\ room with \\ classic game \\ machines, \\ colorful \\ lights, and \\ vintage posters}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_2425453735404758992_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_2425453735404758992_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_2425453735404758992_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_2425453735404758992_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_2425453735404758992_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_2425453735404758992_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Jungle-themed \\ break room with \\ plants, natural \\ wood furniture, \\ and tropical \\ decor}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4336440483597926783_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4336440483597926783_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4336440483597926783_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4336440483597926783_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4336440483597926783_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_4336440483597926783_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Medieval tavern \\ with wooden \\ tables, stone \\ walls, and \\ candle lighting}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6792325757249564920_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6792325757249564920_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6792325757249564920_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6792325757249564920_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6792325757249564920_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6792325757249564920_ours.jpg}
    % \\


    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Victorian \\ parlor with \\ ornate \\ furniture, dark \\ wallpaper, and \\ chandeliers}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_3917677443825827236_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_3917677443825827236_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_3917677443825827236_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_3917677443825827236_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_3917677443825827236_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_3917677443825827236_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{1950s \\ diner-style \\ lounge with \\ checkered \\ floors, red \\ vinyl seats, \\ and jukebox}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_7607527627453949069_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_7607527627453949069_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_7607527627453949069_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_7607527627453949069_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_7607527627453949069_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_7607527627453949069_ours.jpg}
    % \\

    \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Modern art \\ studio with \\ paint \\ splatters, \\ canvases, and \\ abstract \\ sculptures}}}}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6124102173073698624_original.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6124102173073698624_gaussctrl.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6124102173073698624_instruct_gs2gs.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6124102173073698624_instruct_nerf2nerf.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6124102173073698624_DGE.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_b_robotics_6124102173073698624_ours.jpg}
    \\

    \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a Fauvism \\ painting of a \\ photo of a \\ conference room \\ with tables and \\ chairs}}}}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_f_conference_2614162896365812929_original.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_f_conference_2614162896365812929_gaussctrl.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_f_conference_2614162896365812929_instruct_gs2gs.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_f_conference_2614162896365812929_instruct_nerf2nerf.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_f_conference_2614162896365812929_DGE.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_f_conference_2614162896365812929_ours.jpg}
    \\

    \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a Hiroshige \\ Utagawa \\ painting of a \\ kitchen}}}}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_h_kitchen_7313597891086098452_original.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_h_kitchen_7313597891086098452_gaussctrl.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_h_kitchen_7313597891086098452_instruct_gs2gs.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_h_kitchen_7313597891086098452_instruct_nerf2nerf.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_h_kitchen_7313597891086098452_DGE.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_h_kitchen_7313597891086098452_ours.jpg}
    \\

    \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a Bastion game \\ style picture \\ of a flat with \\ a bathroom, \\ living room and \\ a kitchen}}}}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_i_bathroom_2463265628774932085_original.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_i_bathroom_2463265628774932085_gaussctrl.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_i_bathroom_2463265628774932085_instruct_gs2gs.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_i_bathroom_2463265628774932085_instruct_nerf2nerf.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_i_bathroom_2463265628774932085_DGE.jpg}
    & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/scannet_i_bathroom_2463265628774932085_ours.jpg}
    \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ robot dinosaur \\ on the road \\ side}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_3038377324408634801_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_3038377324408634801_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_3038377324408634801_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_3038377324408634801_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_3038377324408634801_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_3038377324408634801_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of an \\ ostrich at a \\ farm}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_an_ostrich_at_a_farm_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_an_ostrich_at_a_farm_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_an_ostrich_at_a_farm_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_an_ostrich_at_a_farm_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_an_ostrich_at_a_farm_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_an_ostrich_at_a_farm_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ giraffe on a \\ desert}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_a_giraffe_on_a_desert_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_a_giraffe_on_a_desert_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_a_giraffe_on_a_desert_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_a_giraffe_on_a_desert_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_a_giraffe_on_a_desert_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/blendedmvs_a_photo_of_a_giraffe_on_a_desert_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ giraffe in zoo}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_giraffe_in_zoo_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_giraffe_in_zoo_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_giraffe_in_zoo_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_giraffe_in_zoo_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_giraffe_in_zoo_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_giraffe_in_zoo_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ medieval horse \\ in front of the \\ castle}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_6128427055822205356_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_6128427055822205356_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_6128427055822205356_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_6128427055822205356_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_6128427055822205356_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_6128427055822205356_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ cyberpunk sci \\ robot horse}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_cyberpunk_sci_robot_horse_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_cyberpunk_sci_robot_horse_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_cyberpunk_sci_robot_horse_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_cyberpunk_sci_robot_horse_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_cyberpunk_sci_robot_horse_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_a_photo_of_a_cyberpunk_sci_robot_horse_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Photo of a \\ dinosaur}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Photo_of_a_dinosaur_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Photo_of_a_dinosaur_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Photo_of_a_dinosaur_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Photo_of_a_dinosaur_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Photo_of_a_dinosaur_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_Photo_of_a_dinosaur_ours.jpg}
    % \\


    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Steampunk horse \\ statue with \\ brass gears, \\ pipes, and \\ mechanical \\ parts}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1620797878807124195_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1620797878807124195_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1620797878807124195_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1620797878807124195_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1620797878807124195_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1620797878807124195_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Horse statue \\ made from very \\ large lego \\ bricks in front \\ of a museum}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1883532210605779899_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1883532210605779899_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1883532210605779899_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1883532210605779899_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1883532210605779899_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/gaussctrl_1883532210605779899_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{80s retro car \\ on a neon grid \\ landscape with \\ pink and blue \\ glowing lights}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6784128519023507286_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6784128519023507286_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6784128519023507286_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6784128519023507286_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6784128519023507286_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6784128519023507286_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Monster truck \\ car with \\ oversized \\ wheels and a \\ lifted body}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_5687717264768732369_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_5687717264768732369_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_5687717264768732369_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_5687717264768732369_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_5687717264768732369_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_5687717264768732369_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Tank with \\ treads and \\ heavy armor in \\ a rugged \\ environment}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6799381787614477972_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6799381787614477972_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6799381787614477972_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6799381787614477972_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6799381787614477972_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_6799381787614477972_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{Photo of a tron \\ legacy \\ nightrider neon \\ futuristic \\ night}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_3698942648060598118_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_3698942648060598118_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_3698942648060598118_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_3698942648060598118_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_3698942648060598118_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_3698942648060598118_ours.jpg}
    % \\

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a photo of a \\ Batmobile}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_photo_of_a_Batmobile_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_photo_of_a_Batmobile_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_photo_of_a_Batmobile_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_photo_of_a_Batmobile_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_photo_of_a_Batmobile_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_photo_of_a_Batmobile_ours.jpg}
    % \\2

    % \raisebox{1.0\height}{\parbox[t]{12mm}{\rotatebox[origin=c]{90}{\makecell{a screenshot of \\ a Minecraft car}}}}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_screenshot_of_a_Minecraft_car_original.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_screenshot_of_a_Minecraft_car_gaussctrl.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_screenshot_of_a_Minecraft_car_instruct_gs2gs.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_screenshot_of_a_Minecraft_car_instruct_nerf2nerf.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_screenshot_of_a_Minecraft_car_DGE.jpg}
    % & \includegraphics[width=0.151\textwidth]{figures/comparisons_figure/raw_jpg_small/bmw_a_screenshot_of_a_Minecraft_car_ours.jpg}
    % \\


\end{tabular}


==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\usepackage{multirow}
\usepackage{array}
\usepackage{vcell}
\usepackage{makecell}
\usepackage{afterpage}
\usepackage{tikz}
\usetikzlibrary{calc}

\newcommand{\red}[1]{{\color{red}#1}}


\definecolor{ms_note}{RGB}{0, 181, 190}
\definecolor{burgundy}{RGB}{150, 0, 0}
\definecolor{pink}{rgb}{1,0.0,1.0}

\definecolor{rgbd_model}{RGB}{180, 96, 6}
\definecolor{warp_controlnet_model}{RGB}{66, 133, 244}
\definecolor{feature_sharing}{RGB}{56, 118, 29}

\newcommand{\ms}[1]{{\color{ms_note}\bf [MS: #1]}}
\newcommand{\zq}[1]{{\color{orange}\bf [ZQ: #1]}}
\newcommand{\jwy}[1]{{\color{purple}\bf [JWy: #1]}}
\newcommand{\jwa}[1]{{\color{green}\bf [JWa: #1]}}
\newcommand{\jp}[1]{{\color{blue}\bf [JP: #1]}}
\newcommand{\todo}[1]{{\color{red} [TODO: #1]}}
\newcommand{\remove}[1]{{\color{pink}\bf [Maybe remove: #1]}}


% --- disable by uncommenting
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


